Data-Driven Superstabilization of Linear Systems under Quantization

This paper focuses on the stabilization and regulation of linear systems affected by quantization in state-transition data and actuated input. The observed data are composed of tuples of current state, input, and the next state's interval ranges based on sensor quantization. Using an established characterization of input-logarithmically-quantized stabilization based on robustness to sector-bounded uncertainty, we formulate a nonconservative infinite-dimensional linear program that enforces superstabilization of all possible consistent systems under assumed priors. We solve this problem by posing a pair of exponentially-scaling linear programs, and demonstrate the success of our method on example quantized systems.

==> sections/abstract_short.tex <==
\begin{abstract}
\label{sec:abstract}
This paper focuses on the stabilization and regulation of linear systems affected by quantization in state-transition data and in actuated input. The observed data are composed of tuples of current state, input, and the next state's interval ranges based on sensor quantization. Using an established characterization of input-logarithmically-quantized stabilization based on robustness to sector-bounded uncertainty, we formulate a nonconservative robust linear program that enforces superstabilization of all possible consistent systems under assumed priors.
We solve this problem by posing a pair of exponentially-scaling linear programs, and demonstrate the success of our method on example systems.

\end{abstract}

==> sections/extensions.tex <==
\section{Extensions}



==> sections/intro_reduced.tex <==
\section{Introduction}
\label{sec:introduction}


This paper performs \ac{DDC} of discrete-time linear systems under data quantization in the state-transition records and logarithmic quantization in the input. Input quantization can be encountered in data-rate constraints for network models when sending instructions to digital actuators, and its presence adds a nonlinearity to system dynamics \cite{brockett2000quantized, elia2001stabilization, nesic2009unified}. 
The logarithmic input quantizer offers the coarsest possible quantization density \cite{elia2001stabilization} among all possible quantization schemes. These logarithmic quantizers admit a nonconservative characterization as a Lur\'{e}-type sector-bounded input \cite{fu2005sector, fu2009finite, zhou2013adaptive}. 
% Subsequent work in \cite{} offers a dynamically gain-updating method to perform logarithmically quantized control in a finite number of quantization intervals (storage).
Data quantization could occur in the storage of sensor data into bits on a computer, and admits the mixed-precision setting of sensor fusion with different per-sensor precisions.

% Quantization in dynamical systems could occur 

% The work in \cite{fu2005sector} is foundational in establishing non

% \urg{Cut down the number of references}

\ac{DDC} is a design method to synthesize control laws directly from acquired system observations and model/noise priors, without first performing  system-identification/robust-synthesis pipeline \cite{HOU20133, hou2017datasurvey}. This paper utilizes a Set-Membership approach to \ac{DDC}: furnishing a controller along with a certificate that the set of all quantized data-consistent plants are contained within the set of all commonly-stabilized plants. Certificate methods for set-membership \ac{DDC} approaches include Farkas certificates for polytope-in-polytope containment \cite{cheng2015robust}, a Matrix S-Lemma for \acp{QMI} to prove quadratic and robust stabilization \cite{waarde2020noisy, van2023quadratic, miller2022lpvqmi}, and Sum-of-Squares certificates of polynomial nonnegativity \cite{dai2020semi, martin2021data, miller2022eiv_short}. 
Other methods for \ac{DDC} include Iterative Feedback Tuning \cite{hjalmarsson1998iterative}, Virtual Reference Feedback Tuning \cite{campi2002virtual, formentin2012non}, Behavioral characterizations (Willem's Fundamental Lemma) with applications to Model-Predictive Control \cite{willems2005note, depersis2020formulas, berberich2021robustmpc}, moment proofs for switching control \cite{dai2018moments}, learning with Lipschitz bounds \cite{lindemann2021learning}, and kernel regression \cite{thorpe2023physicsinformed}.



The most relevant prior work to the quantized \ac{DDC} approach in this paper is the research in \cite{zhao2022data}, which casts quantized control as an 
an $H_\infty$ small-gain task \cite{fu2005sector} and enforces common stabilization over a \iac{QMI} of consistent plants using a Matrix S-Lemma \cite{waarde2020noisy}.
% which utilizes the approach of \cite{fu2005sector} by treating logarithmic-quantizing control as an $H_\infty$ small-gain task. 
% They then formulate the consistency set of data-plants as \iac{QMI}, and use the Matrix S-Lemma 
% \cite{waarde2020noisy} to certify common stabilization. 
In contrast, our work includes individually-quantized data as well as quantized control by developing a polytopic description of the plant consistency set. We then restrict to superstabilization \cite{polyak2001optimal, polyak2002superstable} to formulate \ac{DDC} \acp{LP} over the polytopic consistency set. The \ac{QMI} approach in \cite{zhao2022data} would over-approximate the polytopic consistency constraint with a single ellipsoidal region in the case of data quantization.

% In the case of quantization of data, the \ac{QMI} approach in \cite{zhao2022data} would then over-approximate the polytopic consistency constraint with a single ellipsoidal region.

% \ac{DDC} for quantized systems.


==> sections/quantize_truncation.tex <==
\section{Finite-Dimensional Quantized DDC}
\label{sec:quantize_truncation}

\urg{Show how to solve the quantized LP. Review SOS and Affine-Adjustable Robust Counterparts. We might not do SOS.}
